PASNet: Polynomial Architecture Search Framework for Two-party Computation-based Secure Neural Network Deployment

Two-party computation (2PC) is promising to enable privacy-preserving deep learning (DL). However, the 2PC-based privacy-preserving DL implementation comes with high comparison protocol overhead from the non-linear operators. This work presents PASNet, a novel systematic framework that enables low latency, high energy efficiency & accuracy, and security-guaranteed 2PC-DL by integrating the hardware latency of the cryptographic building block into the neural architecture search loss function. We develop a cryptographic hardware scheduler and the corresponding performance model for Field Programmable Gate Arrays (FPGA) as a case study. The experimental results demonstrate that our light-weighted model PASNet-A and heavily-weighted model PASNet-B achieve 63 ms and 228 ms latency on private inference on ImageNet, which are 147 and 40 times faster than the SOTA CryptGPU system, and achieve 70.54% & 78.79% accuracy and more than 1000 times higher energy efficiency.

==> sections/4_post_training_finetune.tex <==
\subsection{Post Search Training Pipeline}
\label{sec:posttraining}

\subsubsection{Polynomial Architecture Training}
To further enhance the model performance, we adopt the transfer learning method \cite{zhuang2020comprehensive} for general weights initialization and \textbf{STPAI} for polynomial weights. After the appropriate model architecture is found from the NAS framework, we load the pre-trained weight parameters for the backbone model and task to target model architecture. 


\begin{figure} [h]
\centering
\includegraphics[width = 0.8\linewidth]{Fig/Fig_finetune.pdf}
\caption{Fine-grained replacement policy.}
% \cw{(i)For consistency purpose, Organization A, B should be computing server A, B. (ii) I suggest to remove Organization C from the figure.}}
\label{fig:finetune}
% \vspace{-2pt}
\end{figure}

However, we observed that for large models on large datasets, such as ResNet50 on ImageNet, the polynomial function may still lead to instability during the training process. As such, we use a more fine-grained replacement policy shown in Fig.~\ref{fig:finetune}. The replacement ratio $s$ indicates how much the target model layer structure replaces the baseline model layers structure. We follow two iterative steps in training to stabilize the process: parameter update using SGD~\cite{amari1993backpropagation} and s increment.
The experiment shows that the post-search training pipeline, which combines transfer learning, \textbf{STPAI}, and fine-grained replacement policy avoids the gradient explosion and achieves a high model accuracy. 
